Reduced-Precision Strategies for Bounded Memory in Deep Neural Nets

This work investigates how using reduced precision data in Convolutional Neural Networks (CNNs) affects network accuracy during classification. More specifically, this study considers networks where each layer may use different precision data. Our key result is the observation that the tolerance of CNNs to reduced precision data not only varies across networks, a well established observation, but also within networks. Tuning precision per layer is appealing as it could enable energy and performance improvements. In this paper we study how error tolerance across layers varies and propose a method for finding a low precision configuration for a network while maintaining high accuracy. A diverse set of CNNs is analyzed showing that compared to a conventional implementation using a 32-bit floating-point representation for all layers, and with less than 1% loss in relative accuracy, the data footprint required by these networks can be reduced by an average of 74% and up to 92%.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

%

%
In this paper we are interested in alleviating the memory and computation footprint and bandwidth demands of convolutional neural nets. 
In this section we give a brief overview of Convolutional Neural Networks (CNNs).
Neural networks consist of multiple \textbf{layers} and each layer typically comprises multiple computational stages.
Each stage takes data from the previous stage (or input in case of the first layer), 
applies some mathematical operation, sometimes using a parametric function, and produces an estimate of the output in the top layer
%
%
We focus our analysis on image classification, where the goal  of the network is to take an image as input and assign it to one of $K$ classes.
The last layer is typically a softmax, which outputs a set of probabilities over the output space, one for each class. 
%
Traditionally, neural networks utilize fully connected layers, where each of the outputs from the previous layer is connected to all inputs of the next layer. 
%
The weights are found during the training phase typically by minimizing cross-entropy.
%

To reduce the total number of weights and introduce invariances,  convolution layers are often used in lower layers in place of the fully connected layers.
Convolutions operate locally, and the weights are shared across the space. 
%

Neural networks also contain other types of layers such  as non-linear activations (e.g., sigmoid, Rectified Linear Units), local response normalization and pooling.
These layers typically do not use weights, and thus are not "learn," but instead serve to transform data via non-linearities. 
%
%
%
 Most importantly for this work, none of these layers  changes the size of the data.
 The only exception is pooling with stride.
 %
A typical CNN will consist of a series of convolution layers followed by a one or more fully connected layers.
Each convolution and fully connected layer is followed by an activation layer, and sometimes pooling and or  normalization  are employed.

%
%
%
%
%
%
%

 

%

%

%
%

%

\normalsize

%
%

%
%
%
\normalsize

%



%
%

%

%

%
%

%
%
 
%
%
%
%
%
%

%

%
%
%

%


==> sections/compression.tex <==
\subsection{Comparison to Compression}
\label{sec:compression}
The ultimate objective of \OURT is to reduce the quantity of information that has to be transported between the different computing units and the memory elements.
Compression may be used for this purpose as well.
In this section we analyze the compression ratio of two different approaches: \textit{i}) the standard bzip2 that uses the Burrows-Wheeler algorithm\cite{burrows1994block}, and  \textit{ii}) the recently proposed hardware compression technique Base-delta-index compression (B\(\Delta\)I)\cite{Pekhimenko-2012}.
The comparison focuses on the compression ratio that can be achieved.

Figure~\ref{fig:bdi-compr} shows normalized \textit{traffic} over the baseline.
That is the relative size of the total data transferred with compression, and \OURT over the baseline system.
B\(\Delta\)I operates over  blocks of 64 bytes.
For bzip2 we vary the size of the blocks from 256 bytes to 1 KB.
We found that for smaller block sizes bzip2 does not achieve compression.
\OURT is using the configuration reported as optimal for each DNN with an error lower than 0.1\% (see Table~\ref{tab:best_mixed}).

The relative traffic for B\(\Delta\)I varies between 92.2\% for LeNet up to 78.6\% for GoogLeNet.
Bzip2 is worse than B\(\Delta\)I for block sizes of less than or equal to 256 bytes, but achieves higher compression ratios when bigger blocks are used, for 4KB blocks, it achieves a relative traffic of 48\% for GoogLeNet to 73\% for convnet.
\OURT reduces traffic resulting in a relative traffic of as little as 18\% for LeNet and as much as 34\% for NiN.

\begin{figure}
\centering
\includegraphics[scale=0.5]{figs/compression}
\caption{Relative traffic of B\(\Delta\)I, bzip2, and Mixed Precision representation.}
\label{fig:bdi-compr}
\end{figure}



%
%


==> sections/reducing_bw.tex <==
\section{Reducing Off-Chip Memory Traffic}
\label{sec:design}
The variability in the representation length needed by each layer and each network can be exploited to improve performance and energy of DNN implementations.
In this work, we show how it can be used to reduce the data traffic between layers and memory by proposing \OURTL, or \OURT, a layered extension that is compatible with existing DNN implementations.
Figure~\ref{fig:design}a shows a generic DNN compute engine, where on-chip compute units are connected to a memory possibly via an on-chip memory hierarchy.
The compute units can be general purpose processors, graphics processors or  fixed-function accelerators. 

Without loss of generality, we assume that layers read their inputs from memory and write the outputs to memory, and that the memory is off-chip.
This is typical in modern software implementations such as Caffe, implemented over general purpose and graphics processors.
This is a reasonable assumption in general as the amount of data produced and processed by layers often exceeds the on-chip buffering capacity of modern integrated circuits.
Furthermore, even when the layers are spread over multiple chips, there will still be significant data movement for inter-chip communication through the network~\cite{DaDiannao}.

\begin{figure}
\centering
\subfloat[]{\includegraphics[scale=0.19]{figs/design0.pdf}}
\subfloat[]{\includegraphics[scale=0.19]{figs/design1.pdf}} 
\caption{(a)~A Generic DNN compute engine. (b)~Adding conversion layers from and to memory.}
\label{fig:design}
\end{figure}

In the baseline implementation of Figure~\ref{fig:design}(a) a single, pre-selected numerical representation is used when processing the values by the compute units and when storing results in memory.
For example, in a modern graphics processor system, single-precision floating-point may be used for the calculations and when reading and writing data from memory.
Figure~\ref{fig:design}(b) shows \OURT as a layered extension where two representations are now in use: a \textit{computation} and a \textit{storage} representation.
The computation representation is the one used in the original system of part (a).
This representation persists internally and is used for all calculations as before.
The storage representation, which uses fewer bits compared to the computation representation, is used for the data stored in memory.
The storage representation length varies depending on the layer being executed.
When reading data from memory, the numerical values are converted from the storage representation to the computation representation.
Conversely, when writing data out to memory, numerical results are converted from the computation representation to the storage representation.
For example, in a graphics processor system, we may still use single-precision floating-point when performing the calculations internally (computation representation), but use a shorter, fixed-point representation when storing to memory (storage representation).
Using two different representations for computations and storage allows \OURT to be implemented as a layered extension over existing compute engine implementations.
Since the storage representation uses fewer bits some precision is lost during the conversion.
However, we have seen that DNNs are tolerant to such precision loss.
Future work may consider reducing the representation in the compute units as well.
For the rest of this discussion we assume that the computation representation is single-precision floating-point and the storage representation is fixed-point.

Using fixed-point representations for both computations and storage has been considered before for DNNs.
The innovation here is that: 1) we allow the storage representation to vary, and 2) we allow for a different per layer storage representation.
These choices enable further reductions in memory footprint and traffic compared to existing systems that have to use a single representation that will work well for all possible networks.
We assume that the DNN has been annotated with information about the representation that ought to be used per layer.
That is, how many bits should be used for the integer and fractional portions of the fixed-point representation for each layer.
This information can be associated with the address ranges that contain the data values and weights used by the network or it could be encoded in the memory instructions.
Given that networks have relatively few layers, and that the layers process and produce a few large continuous arrays, a small software-managed hardware table in the conversion units is sufficient for informing the hardware conversion units which memory reads and writes can be converted. 

The conversion can be done at the level of individual memory accesses or at the level of cache blocks.
For example, for a graphics processor it could either be done at the level of the cache block used by the compute engines on fill (to reduce hit time) or upon access to a line (to increase effective cache capacity).
Either way, the key benefit from the conversion is that the amount of data transferred to and from memory is reduced.
This reduces the energy used by the memory subsystem.
Another indirect yet important benefit is that for a given amount of memory it increases the size of DNNs that can be processed.
Today, memory footprint is seen as the main limiter in DNN processing during classification~\cite{goingdeeper14}.
Even when on-chip buffers are used to reduce off-chip traffic, our proposed extension can be used to reduce the amount of data that has to be communicated on chip and to effectively boost the capacity of these buffers.
It is well understood that in modern semiconductor technologies, data movement energy tends to dominate compute energy with off-chip accesses being 2-3 orders of magnitude more expensive than a floating-point addition or multiplication~\cite{sameh}.

Conversion between floating-point and fixed point is relatively straightforward~\cite{DallyHarting2012}, more so for our application where the maximum length of the fixed-point representation needed in practice is limited to less than 16 bits.
A final shifting stage can pack several of these fixed point numbers into a memory block for writing to memory.
Previous research showed the feasibility of a cache memory design that uses blocks of multiple sizes~\cite{amoeba,adjustable}.
Since the DNN produces several blocks at the time, except for the last few blocks, we are guaranteed to have a continuous stream of blocks being delivered from the units for coalescing.
Writes are off the critical path.
While conversion may increase read latency, this increase will be a tiny fraction of the off-chip latency.
Moreover, DNNs exhibit massive data parallelism and thus their execution is latency tolerant.
This is confirmed experimentally in Section~\ref{sec:evaluation}.

